Object Handovers: a Review for Robotics

This article surveys the literature on human-robot object handovers. A handover is a collaborative joint action where an agent, the giver, gives an object to another agent, the receiver. The physical exchange starts when the receiver first contacts the object held by the giver and ends when the giver fully releases the object to the receiver. However, important cognitive and physical processes begin before the physical exchange, including initiating implicit agreement with respect to the location and timing of the exchange. From this perspective, we structure our review into the two main phases delimited by the aforementioned events: 1) a pre-handover phase, and 2) the physical exchange. We focus our analysis on the two actors (giver and receiver) and report the state of the art of robotic givers (robot-to-human handovers) and the robotic receivers (human-to-robot handovers). We report a comprehensive list of qualitative and quantitative metrics commonly used to assess the interaction. While focusing our review on the cognitive level (e.g., prediction, perception, motion planning, learning) and the physical level (e.g., motion, grasping, grip release) of the handover, we briefly discuss also the concepts of safety, social context, and ergonomics. We compare the behaviours displayed during human-to-human handovers to the state of the art of robotic assistants, and identify the major areas of improvement for robotic assistants to reach performance comparable to human interactions. Finally, we propose a minimal set of metrics that should be used in order to enable a fair comparison among the approaches.

==> arxiv_page.tex <==
\onecolumn
{\Huge  \bf IEEE Copyright Notice}
\newline
\newline
\textcopyright 2020 IEEE. Personal use of this material is permitted.  Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting\slash republishing this material for advertising or promotional purposes, creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component of this work in other works.
\newline
\newline
The work has been submitted to IEEE Transactions on Robotics (T-RO) in July 2020.

==> conclusions_old.tex <==
\section{\textcolor{blue}{Challenges and future work}}
\label{sec:conc}

In this paper, we analyse in detail the two phases of a handover, reviewing the results from human studies and the corresponding state of the art in the robotic literature. \st{We summarise the salient features of the papers implementing physical human-robot handovers in Table~I.} \hl{At this point, we focus our analysis on human-robot handover papers that present novelty in any of the aspects of the two phases (pre-handover and physical handover) and that include experiments with a real robot. A panoramic view of these contributions can be found in Table~I.} For each paper we report: the paradigm (robot-to-human or human-to-robot); what the authors investigated (communication, grasping, motion planning and control, and perception during the pre-handover phase; grip force and error handling during the physical handover); whether the handover location was fixed, pre-planned accounting for aspects such as the ergonomics, or adapted online to the human partner; whether the experimental protocol included a post-handover task for the receiver; the metrics used to assess the task performance and the user experience; and finally the number of different objects used in the real robot experiments.

\hl{In order to bridge the gap between human-human handovers and human-robot handovers, there are a number of open challenges to conquer. First of all, the interaction should become more fluid and fluent. Secondly, the agents should communicate and collaborate more naturally, changing their behaviour to accommodate their partner. In most instances, robots present predefined behaviours that force the human partner to comply. This not only decreases the perceived alliance of the robot, but makes the joint action less natural. Finally, we believe that experimental protocols should be more stardandised, in order to allow a fairer comparison among the proposed algorithms, methods and approaches. Next subsections highlight the most important research directions to address those challenges.} 

\subsection{\textcolor{blue}{Safety}}
\hl{Safety is the condicio sine qua non HRI would not be possible. Every handover must first be a safe interaction. In} Sect.\ref{sec:safety} \hl{ciao}

\subsection{Adaptability and Handover Location}
Studies in neuroscience, physiology and psychology highlight that a handover is an intricate joint action that requires a physical level and a cognitive coordination. In particular, it seems apparent that the cognitive level of the interaction is as important as the physical level \cite{Lemaignan2014}, for a robot to be considered as a partner, and not only as a tool \cite{Breazel2004}. To match the human skills of understanding and adaptation \cite{Edsinger2007}, it is preferable that robots also display adaptation and understanding. In fact, human givers can control the object's position and orientation to facilitate the robotic receiver's grasping of the object \cite{Edsinger2007}. However, fatigue of the human worker having to accommodate the robot repeatedly and for a long time can become an issue \cite{Peternel2019}. From this perspective, robots that are able to adopt different behaviours adapting to their partner could assist their human counterpart \cite{Koene2014, Huang2015}. 
%To this end, pure planning is not sufficient, as the subjective perception of a good interaction depends more on the adaptation of the robot than on the sheer performance of the robot. 
In other words, it is crucial to account for the feedback coming from the human partner during the interaction when controlling the robot. However, as can be seen in Table 1, to date most approaches focus on fixed or pre-planned handover locations, with far fewer attempts at adapting to the human partner online. In many human-robot handover scenarios, the handover location is kept fixed, \textit{i.e.}, the robot is either going always to the same position for the object transfer, or the handover location is pre-planned based on several criteria (including ergonomics, safety, etc) and not updated in real-time with the perceptual feedback. This is far from ideal, as the human has to potentially adapt to the robot and could incur cognitive and physical fatigue. The ergonomics of the interaction should be accounted for, as the transfer should happen in the comfort zone of the human, \textit{i.e.}, the range of positions (and tasks to perform in) reachable (and doable) with little or no compensatory movements \cite{Kolsch2003}. In humans, an optimisation principle over a muscle stress index is shown to determine the arm motions and postures (selected over the infinite possibilities of motion) and also the perceived comfort \cite{Katayama2003}. We believe that while pre-planning such a location accounting for the ergonomics and the physical characteristics of the human partner is appropriate, more effort is needed in order to adjust to changing circumstances (adapting in real-time to the needs of the human partner). 


\subsection{Communication}
Communication is a key factor to achieve a successful coordination during a joint action. Humans use speech, gaze, and body movements to communicate intent and coordinate during the execution of the joint action. We observe that robots have displayed a general lack of communication skills for object handovers.  Most of the effort in the literature so far has been put on the physical aspects of the interaction, focusing on motion planning and control, grasping and perception. 
%However, task-oriented grasping is an aspect that in our opinion deserves and calls for more effort. 
On the other hand, effort in communication is less prevalent, \textcolor{red}{as only 37\% of the papers in Table~I include an element of communication in their implementation.} 
%A huge effort is needed on the cognitive layer. For example, 
\hl{We believe that improving the communication cues provided to the human partner by the robot is a key factor to increase the naturalness and fluency of human-robot handovers. }

\subsection{Grip Release}
There are also only a few papers that focus on grip release and how to handle potential falls of the object. While the literature in human studies continues to investigate how both agents modulate their grip force on the object and how the different sensory modalities (vision and tactile) come into play, most of the reviewed work has adopted a simplistic approach, \textit{i.e.}, robotic givers completely release the object whenever a pull by the receiver is detected. Conversely, robotic receivers need to modulate their pulling force as too little force could be unsafe for the object transfer and too much force could be dangerous for the human partner. We believe that grip force modulation is a key component that needs further investigation and effort. There are many additional open research directions, such as: (i) the use of different hardware (under-actuated vs fully actuated, soft vs rigid, parallel jaw gripper vs multi-fingered hands); (ii) the use of different grasping strategies (grasp type and location on the object); and (iii) the use of objects varying their size and weight. Such exploration could thus give rise to various options to modulate the grip. 

\subsection{Paradigm}
In terms of the paradigm, Robot-to-Human (R2H) handovers have been more frequently investigated (\textcolor{red}{87\% of surveyed papers in Table~I}), compared to Human-to-Robot (H2R) (\textcolor{red}{29\%}), \textcolor{red}{while only 16\% reported experiments in both directions}. We speculate that the idea of having a robot assistant that can fetch objects and give them to humans when needed, has driven the deeper investigation of the R2H paradigm. The R2H paradigm is particularly representative of the cases where the human receiver will then perform a cognitively challenging task with the object, a task that robots are not yet able to perform. However, it is our opinion that H2R handovers are worth exploring more and represent an open area of research. One of the biggest challenges in human-to-robot handovers is safety \cite{Rosenberger2020}, as the robot should be careful to not contact the human giver. For this to happen, perception systems should be able to robustly discriminate the human giver (hand and arm) from the object \cite{Yang2020, Rosenberger2020}. Moreover, in the H2R paradigm grasp planning becomes another critical issue, as the robot will have to perform a task with the handed-over object, \textit{i.e.}, at the very least need to put the object down in a pose preferable to humans \cite{newbury2020learning}. 

\subsection{Role of the Task}
From the robot's higher-level behaviour standpoint, there is a critical need for improvement in the integration of cognitive and physical reasoning \cite{Pandey2014} in both paradigms (H2R and R2H). In other words,  robots currently lack a vision and understanding of the general goal of such an action. Such understanding is the key contributor to enabling higher-order planning \cite{Gonzalez2011, Rosenbaum2012, Meyer2013, Cini2019}.
For example, robotic grasping has achieved peaks in performance
\cite{Morrison2019} \cite{Adjigble2018}
\cite{Roa2009}
\cite{Levine2018}; however, the ultimate goal of the grasp is rarely taken into account \cite{Ortenzi2019}. As a result, robots can manage to grasp objects but seldom these grasps would allow the execution of a task with the objects. Considering a handover, a successful grasp should account for the interaction partner and this is a key feature that a robot should display in order to be fully collaborative. 

Following a similar reasoning, we believe that any experimental protocol should include a task to perform by the receiver with the handed-over object, as proposed in \cite{Cini2019}. This is a critical consideration because the object exchange is normally initiated in order for the receiver to perform a task with the handed-over object. 
%For this reason, we consider this phase to be part of a broader definition of a handover. A stricter definition could consider the end of the physical object exchange as the end of the joint action. 
A complete experimental procedure should consider the capability of the receiver to use the object directly following the handover. If the receiver can grasp the object in a way that its subsequent use does not require any further in-hand or bi-manual re-manipulation, then the receiver can start the task straight away after the physical exchange of the object. 
Conversely, the receiver might need to re-adjust their grasp of the object in case their temporary grasp (realised during the exchange) is not an ideal grasp to correctly use the object for the specific task.
However, this post-handover grasp adjustment could decrease the quality of the handover in objective terms (longer task performance time, higher strain when the handover happens multiple times) and in subjective terms (the giver could be perceived as a lesser partner, and the task could be perceived as more cognitively difficult). These quality evaluations are pivotal in establishing the degree of success of a handover, as considered in the Section \ref{sec:metrics} on metrics. However, very few experimental protocols include a posterior task for the receiver (\textcolor{red}{18\% of the surveyed papers}). Even though it might be argued that a handover can be considered finished after the object transfer, we believe that such task performance is important to effectively assess the overall performance of the dyad and gauge the experience of the human partner, particularly for the R2H paradigm. 

\subsection{Proposed Set of Metrics}
Our survey has revealed a need for standardisation in the choice of metrics and objects for real robot experiments. Most of the surveyed papers in Table~I report results using task performance metrics (\textit{e.g.}, success rate and timings) and subjective metrics on the experience of the human partner (often in the form of Likert-scale post-experiment questionnaires). The last three rows of the table report papers that focus purely on metrics that have been used for handovers. We believe that a minimal set of metrics should be defined in order to enable a fairer and more direct comparison among the different approaches. To this end, we propose the following combination of metrics that assess the most common aspects of a handover: 
\begin{enumerate}
    \item Task performance (objective): success rate, total handover time, receiver's task completion time.
    \item Experience of the human (subjective): fluency, trust in robot, working alliance.
\end{enumerate}
This minimal set includes metrics which are clearly defined, thus reproducible, and which are easy to measure. For these reasons, the set does not include psycho-physiological measurements as they require sensors placed on the body of the human participant, and thus are difficult to standardise and deploy in a variety of contexts. 

The experience of the human participant should be assessed administering the following questionnaire (the following set of questions includes a subset of questions from \cite{Hoffman2019}):
\begin{enumerate}
    \item Human-Robot Fluency 
    \begin{itemize}
        \item The human-robot team worked fluently together.
        \item The human-robot team's fluency improved over time.
        \item The robot contributed to the fluency of the interaction.
    \end{itemize}
    \item Trust in Robot 
    \begin{itemize}
        \item I trusted the robot to do the right thing at the right time.
        \item The robot was trustworthy.
        %\item The robot trusted me to do the right thing at the right time. 
    \end{itemize}
    \item Working Alliance 
    \begin{itemize}
        \item The robot accurately perceives what my goals are.
        %\item The robot does not understand what I am trying to accomplish (R).
        \item I understand what the robot's goals are.
        %\item I do not understand what the robot is trying to accomplish (R).
        \item The robot and I are working towards mutually agreed upon goals.
    \end{itemize}
\end{enumerate}
All questions should be evaluated on a Likert scale.
%(R) indicates reverse scale.
%Cronbach's $\alpha$ should also be reported ADD WHAT ALPHA MEANS/ADD. 
We believe that this set of questions covers a broad set of important general aspects of the interaction, namely fluency, trust and working alliance. Furthermore, additional questions can be added to this minimal set in order to investigate additional specific aspects of a handover, such as preference between different approaches, and learning/improvement over time.

\subsection{Objects}
\textcolor{red}{68\% of the surveyed papers in Table~I used only a single object class and only 10\% of the papers used four or more object classes.} This observation shows that generalisation of handovers to a variety of objects has not been the main focus of a majority of the papers until very recently \cite{Rosenberger2020}. The most commonly used test objects have been either cylindrical objects such as bottles (\textcolor{red}{55\% of the surveyed work) and rectangular objects such as boxes (26\% of the surveyed work)}. This is likely because these object shapes are easier to grasp and many everyday objects belong to those categories. 
We support the practice of a broader set of objects, as different objects generate different behaviours and can be used to address different manipulation tasks. We propose the use of objects that elicit all three grasp macro-types in \cite{Cutkosky1989}, \textit{i.e.}, power, intermediate and precision grasps. The three macro-types offer sufficient opportunities to explore different behaviours, investigating aspects such as different object offering and reception; different post-handover tasks; and handover of objects with different weights and shapes. 
%To this end, we propose the use of the following objects in handover experiments:
%\begin{enumerate}
%\item a cylindrical object such as a water bottle;
%\item a rectangular object such as a box;
%\item at least one selected item from ``Food" and ``Kitchen" objects from the YCB object dataset \cite{Calli2015a}.
%\end{enumerate}
Nevertheless, we acknowledge that the choice of objects might depend on the specific focus of each study. For example, studies on the reaching motion might place their focus on the motion and not on the objects, so three objects evoking the three grasp types would be enough. However, studies more focused on the objects, such as a study on object orientation in the preparation to hand over, would require a wider set of experimental objects.

Our proposition of a minimal set of metrics and of objects to use in an experimental protocol is targeted to increase the possibility of fair comparison among the approaches. A handover is a sophisticated joint action that includes many different aspects (communication, planning, grip release, etc). For this reason, there has been a general non-uniformity in protocols and metrics. We believe that our proposition of metrics and objects covers the most common aspects of a handover, thus enabling a fair comparison among approaches, while allowing for additions when the research questions call for investigation into more specific aspects.

==> src/table_old.tex <==
\begin{landscape}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{D0CECE} 
\multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}  & \multicolumn{4}{c}{\cellcolor[HTML]{D0CECE}Pre-Handover}    & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{2}{c}{\cellcolor[HTML]{D0CECE}Physical Handover}    & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}      & \multicolumn{3}{c}{\cellcolor[HTML]{D0CECE}Metric}   \\
\rowcolor[HTML]{D0CECE} 
\multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}  & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}  & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}    & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}    & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}      & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}      & \multicolumn{2}{c}{\cellcolor[HTML]{D0CECE}Experience of the human} \\
\rowcolor[HTML]{D0CECE} 
\multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}Year}} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}Paper}}     & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}Paradigm}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Comm.}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Grasping}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Motion}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Perception}} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Handover\\Location\end{tabular} }} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Physical\\Handover\end{tabular} }} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Grip Force}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Error\\Handling\end{tabular}}} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Post-HO\\Task\end{tabular} }} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Overall\\performance\end{tabular}}} & Quantitative     & Qualitative    \\
\hline
%1997  & Agah et al. \cite{Agah1997} & R2H &  &  & \checkmark & \checkmark& Not-fixed  &  &  &  &  &  & & \\
%\hline
2007  & Edsinger et al. \cite{Edsinger2007} & H2R \& H2R & \checkmark& \checkmark & \checkmark & \checkmark& Fixed & \checkmark &  &  &  & \checkmark & & \\
\hline
2009  & Choi et al. \cite{Choi2009} & R2H & & & \checkmark & \checkmark& Not-fixed  & \checkmark &  &  &  & \checkmark &  & \checkmark  \\
\hline
2009  & Huber et al. \cite{Huber2009a}  & R2H  &  & & \checkmark  &  & Fixed  & \checkmark& & & & & & \checkmark\\
\hline
2010  & Sisbot et al. \cite{Sisbot2010} & R2H &  & & \checkmark & \checkmark& Not-fixed  & \checkmark &  &  &   & &  &  \\
\hline
2011  & Dehais et al. \cite{Dehais2011}  & R2H   &   & & \checkmark  & \checkmark& Fixed  & \checkmark &  &  &  &  & \checkmark & \checkmark\\
\hline
2011  & Cakmak et al. \cite{Cakmak2011a} & R2H  & & & \checkmark  & \checkmark& Not-fixed & \checkmark &  &  &  &  &  & \checkmark  \\
\hline
2011  & Cakmak et al. \cite{Cakmak2011b} & R2H & \checkmark& & \checkmark  & \checkmark& Fixed  & \checkmark &  &  &  & \checkmark &  & \checkmark  \\
\hline
2011  & Micelli et al. \cite{Micelli2011} & H2R  & & \checkmark & \checkmark& \checkmark& Not-fixed  & \checkmark &  &  &  & \checkmark & & \checkmark  \\
\hline
2011  & Bohren et al. \cite{Bohren2011} & R2H   &   & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &   &   & \checkmark  &   &  \\
\hline
2012  & Mainprice et al. \cite{Mainprice2012} & R2H   &   & & \checkmark  & \checkmark& Fixed  & \checkmark   &  &    &  & \checkmark    &     & \checkmark  \\
\hline
2012  & Aleotti et al. \cite{Aleotti2012}  & R2H   &   & \checkmark   & \checkmark  & \checkmark& Fixed  & \checkmark &   &    &  & \checkmark  &     & \checkmark  \\
\hline
2013  & Chan et al. \cite {Chan2013}  & R2H   &   & & \checkmark  &  & Fixed  & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2013  & Shi et al. \cite{Shi2013}   & R2H   & \checkmark & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    &     &    \\
\hline
2013  & Yamane et al. \cite {Yamane2013}  & H2R   &   & & \checkmark  & \checkmark& Unclear & \checkmark   &  &    &      &      &     &    \\
\hline
2013  & Strabala et al. \cite{Strabala2013}  & R2H \& H2R  & \checkmark & & \checkmark  & \checkmark& Not-fixed   & \checkmark & \checkmark&    &   & \checkmark   &     & \checkmark  \\
\hline
2013  & Grigore et al. \cite{Grigore2013}      & R2H   & \checkmark & & \checkmark  & \checkmark& Fixed  & \checkmark   &  &    &      & \checkmark    &     &    \\
\hline
2014  & Aleotti et al. \cite{Aleotti2014}      & R2H   & \checkmark & \checkmark   & \checkmark  & \checkmark& Fixed  & \checkmark   &  &    &      & \checkmark    &     & \checkmark  \\
\hline
2014  & Moon et al. \cite{Moon2014}  & R2H   & \checkmark & &    &  & Fixed  & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2014  & Aleotti et al. \cite{Aleotti2014}      & R2H   & \checkmark & \checkmark   & \checkmark  & \checkmark& Fixed  & \checkmark   &  &    &      & \checkmark    &     & \checkmark  \\
\hline
2014  & \begin{tabular}[x]{@{}c@{}c@{}}Koene  et al. \cite{Koene2014},\\Prada et al. \cite{Prada2014}, \\Koene et al. \cite{Koene2014b}\end{tabular}  & H2R \& H2R     & \checkmark & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2014  & Chan et al. \cite{Chan2014}  & R2H   &   & & \checkmark  & \checkmark& Fixed  & \checkmark   & \checkmark&    &      & \checkmark    &     &    \\
\hline
2014  & Admoni et al. \cite{Admoni2014}       & R2H   & \checkmark & & \checkmark  & \checkmark& Fixed  & \checkmark   & \checkmark&    & \checkmark    & \checkmark    &     & \checkmark  \\
\hline
2015  & Suay et al. \cite{Suay2015}  & R2H   &   & & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    & \checkmark   &    \\
\hline
2015  & Huang et al. \cite{Huang2015}  & R2H   & \checkmark & &    & \checkmark& Fixed  & \checkmark   &  &    &      & \checkmark    &     & \checkmark  \\
\hline
2016  & Parastegari et al. \cite{Parastegari2016}  & R2H   &   & &    & \checkmark& Fixed  & \checkmark   & \checkmark& \checkmark  &      & \checkmark    &     & \checkmark  \\
\hline
2016  & Maeda et al. \cite{Maeda2016}  & R2H   &   & & \checkmark  & \checkmark& Unclear & \checkmark   &  &    & \checkmark    & \checkmark    &     &    \\
\hline
2016  & Vahrenkamp et al. \cite{Vahrenkamp2016}   & R2H \& H2R     &   & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    &     &    \\
\hline
2016  & Kupcsik et al. \cite{Kupcsik16}      & R2H   &   & & \checkmark  & \checkmark& Not-fixed    & \checkmark   & \checkmark&    &      &      &     & \checkmark  \\
\hline
2016  & Medina et al. \cite{Medina2016}       & R2H   &   & & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    &     &    \\
\hline
2017  & Gomez Eguıluz et al. \cite{Gomez2017} & R2H & &  & & & Fixed & \checkmark& \checkmark& \checkmark &  & \checkmark&  &  \\
\hline
2017  & Bestick et al. \cite{Bestick2017}      & R2H   &   & \checkmark   & \checkmark  &  & \cellcolor[HTML]{FFFFFF}Fixed      & \checkmark   &  &    & \checkmark    & \checkmark    &     & \checkmark  \\
\hline
2017  & Peternel et al. \cite{Peternel2017}     & R2H   &   & & \checkmark  &  & Fixed  & \checkmark   &  &    &      &      & \checkmark   &    \\
\hline
2017  & Konstantinova et al. \cite{Konstantinova2017}      & R2H \& H2R     &   & &    &  & Unclear & \checkmark   & \checkmark&    &      & \checkmark    &     &    \\
\hline
2018  & Controzzi et al. \cite{Controzzi2018}    & R2H   &   & &    &  & Fixed  & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2018  & Pan et al.  \cite {Pan2018}   & H2R   & \checkmark & \checkmark   & \checkmark  & \checkmark& \cellcolor[HTML]{FFFFFF}Not-fixed    & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2020      & Yang et al.  \cite {Yang2020}  & H2R   &   & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    &     & \checkmark  \\
\hline
2020      & Rosenberger et al.  \cite {Rosenberger2020}  & H2R   &   & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  & \checkmark    &      & \checkmark    &     &   \\
\hline
\rowcolor[HTML]{E7E6E6} 
2006      & Kulic et al. \cite{Kulic2006}  & N/A   &   & & \checkmark  &  &     &     &  &    &      &      & \checkmark   & \checkmark  \\
\hline
\rowcolor[HTML]{E7E6E6} 
2009      & Bartneck et al. \cite{Bartneck2009}      & N/A   &   & &    &  &     &     &  &    &      &      &     & \checkmark  \\
\hline
\rowcolor[HTML]{E7E6E6} 
2019      & Hoffman \cite{Hoffman2019}    & N/A   &   & &    &  &     &     &  &    &      & \checkmark    &     & \checkmark \\
\hline
\end{tabular}
\caption{Comparison of the papers presenting novelty about human-robot handovers and experiments with a real system. This table reports: the paradigm (robot-to-human R2H or human-to-robot H2R); the aspects of the pre-handover phase under investigation (communication, grasping, motion planning and control, perception); whether the handover location was fully pre-planned (fixed) or adapted online (not-fixed); whether during the physical handover, grip force was regulated and error handling dealt with; whether the experimental protocol foresaw a post-handover task. Finally, we report whether the reported results are based on metrics encompassing the overall performance, and a quantitative and qualitative assessment of the experience of the human partner. The last three entries are papers purely investigating the metrics for a handover.}
\end{table}
\label{table:comparison}
\end{landscape}

==> table.tex <==
\begin{landscape}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{D0CECE} 
\multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{2}{c}{\cellcolor[HTML]{D0CECE}Paradigm} & \multicolumn{4}{c}{\cellcolor[HTML]{D0CECE}Pre-Handover}    & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{2}{c}{\cellcolor[HTML]{D0CECE}Physical Handover}    & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}      & \multicolumn{3}{c}{\cellcolor[HTML]{D0CECE}Metric}   \\
\rowcolor[HTML]{D0CECE} 
\multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{2}{c}{\cellcolor[HTML]{D0CECE}}  & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}  & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}    & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}     & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}   & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}    & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}      & \multicolumn{1}{c}{\cellcolor[HTML]{D0CECE}}      & \multicolumn{2}{c}{\cellcolor[HTML]{D0CECE}Experience of the human} \\
\rowcolor[HTML]{D0CECE} 
\multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}Year}} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}Paper}}     & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}R2H}} &
\multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}H2R}} &
\multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Comm.}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Grasping}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Motion}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Perception}} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Handover\\Location\end{tabular} }} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Physical\\Handover\end{tabular} }} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}Grip Force}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Error\\Handling\end{tabular}}} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Post-HO\\Task\end{tabular} }} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0CECE}\begin{tabular}[x]{@{}c@{}}Overall\\performance\end{tabular}}} & Quantitative     & Qualitative    \\
\hline
%1997  & Agah et al. \cite{Agah1997} & R2H &  &  & \checkmark & \checkmark& Not-fixed  &  &  &  &  &  & & \\
%\hline
2007  & Edsinger et al. \cite{Edsinger2007} & \checkmark & \checkmark & \checkmark& \checkmark & \checkmark & \checkmark& Fixed & \checkmark &  &  &  & \checkmark & & \\
\hline
2009  & Choi et al. \cite{Choi2009} & \checkmark & & & & \checkmark & \checkmark& Not-fixed  & \checkmark &  &  &  & \checkmark &  & \checkmark  \\
\hline
2009  & Huber et al. \cite{Huber2009a}  & \checkmark &  &  & & \checkmark  &  & Fixed  & \checkmark& & & & & & \checkmark\\
\hline
2010  & Sisbot et al. \cite{Sisbot2010} & \checkmark & &  & & \checkmark & \checkmark& Not-fixed  & \checkmark &  &  &   & &  &  \\
\hline
2011  & Dehais et al. \cite{Dehais2011}  & \checkmark &   &   & & \checkmark  & \checkmark& Fixed  & \checkmark &  &  &  &  & \checkmark & \checkmark\\
\hline
2011  & Cakmak et al. \cite{Cakmak2011a} & \checkmark &  & & & \checkmark  & \checkmark& Not-fixed & \checkmark &  &  &  &  &  & \checkmark  \\
\hline
2011  & Cakmak et al. \cite{Cakmak2011b} & \checkmark & & \checkmark& & \checkmark  & \checkmark& Fixed  & \checkmark &  &  &  & \checkmark &  & \checkmark  \\
\hline
2011  & Micelli et al. \cite{Micelli2011} & & \checkmark  & & \checkmark & \checkmark& \checkmark& Not-fixed  & \checkmark &  &  &  & \checkmark & & \checkmark  \\
\hline
2011  & Bohren et al. \cite{Bohren2011} & \checkmark &   &   & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &   &   & \checkmark  &   &  \\
\hline
2012  & Mainprice et al. \cite{Mainprice2012} & \checkmark &   &   & & \checkmark  & \checkmark& Fixed  & \checkmark   &  &    &  & \checkmark    &     & \checkmark  \\
\hline
2012  & Aleotti et al. \cite{Aleotti2012}  & \checkmark &   &   & \checkmark   & \checkmark  & \checkmark& Fixed  & \checkmark &   &    &  & \checkmark  &     & \checkmark  \\
\hline
2013  & Chan et al. \cite {Chan2013}  & \checkmark &   &   & & \checkmark  &  & Fixed  & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2013  & Shi et al. \cite{Shi2013}   & \checkmark &   & \checkmark & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    &     &    \\
\hline
2013  & Yamane et al. \cite {Yamane2013}  & & \checkmark   &   & & \checkmark  & \checkmark& Unclear & \checkmark   &  &    &      &      &     &    \\
\hline
2013  & Strabala et al. \cite{Strabala2013}  & \checkmark & \checkmark  & \checkmark & & \checkmark  & \checkmark& Not-fixed   & \checkmark & \checkmark&    &   & \checkmark   &     & \checkmark  \\
\hline
2013  & Grigore et al. \cite{Grigore2013}      & \checkmark &   & \checkmark & & \checkmark  & \checkmark& Fixed  & \checkmark   &  &    &      & \checkmark    &     &    \\
\hline
2014  & Aleotti et al. \cite{Aleotti2014}      & \checkmark &   & \checkmark & \checkmark   & \checkmark  & \checkmark& Fixed  & \checkmark   &  &    &      & \checkmark    &     & \checkmark  \\
\hline
2014  & Moon et al. \cite{Moon2014}  & \checkmark &   & \checkmark & &    &  & Fixed  & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2014  & Aleotti et al. \cite{Aleotti2014}      & \checkmark &   & \checkmark & \checkmark   & \checkmark  & \checkmark& Fixed  & \checkmark   &  &    &      & \checkmark    &     & \checkmark  \\
\hline
2014  & \begin{tabular}[x]{@{}c@{}c@{}}Koene  et al. \cite{Koene2014},\\Prada et al. \cite{Prada2014}, \\Koene et al. \cite{Koene2014b}\end{tabular}  & \checkmark & \checkmark   & \checkmark & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2014  & Chan et al. \cite{Chan2014}  & \checkmark &   &   & & \checkmark  & \checkmark& Fixed  & \checkmark   & \checkmark&    &      & \checkmark    &     &    \\
\hline
2014  & Admoni et al. \cite{Admoni2014}       & \checkmark &   & \checkmark & & \checkmark  & \checkmark& Fixed  & \checkmark   & \checkmark&    & \checkmark    & \checkmark    &     & \checkmark  \\
\hline
2015  & Suay et al. \cite{Suay2015}  & \checkmark &   &   & & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    & \checkmark   &    \\
\hline
2015  & Huang et al. \cite{Huang2015}  & \checkmark &   & \checkmark & &    & \checkmark& Fixed  & \checkmark   &  &    &      & \checkmark    &     & \checkmark  \\
\hline
2016  & Parastegari et al. \cite{Parastegari2016}  & \checkmark &   &   & &    & \checkmark& Fixed  & \checkmark   & \checkmark& \checkmark  &      & \checkmark    &     & \checkmark  \\
\hline
2016  & Maeda et al. \cite{Maeda2016}  & \checkmark &   &   & & \checkmark  & \checkmark& Unclear & \checkmark   &  &    & \checkmark    & \checkmark    &     &    \\
\hline
2016  & Vahrenkamp et al. \cite{Vahrenkamp2016}   & \checkmark & \checkmark     &   & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    &     &    \\
\hline
2016  & Kupcsik et al. \cite{Kupcsik16}      & \checkmark &   &   & & \checkmark  & \checkmark& Not-fixed    & \checkmark   & \checkmark&    &      &      &     & \checkmark  \\
\hline
2016  & Medina et al. \cite{Medina2016}       & \checkmark &   &   & & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    &     &    \\
\hline
2017  & Gomez Eguıluz et al. \cite{Gomez2017} & \checkmark & & &  & & & Fixed & \checkmark& \checkmark& \checkmark &  & \checkmark&  &  \\
\hline
2017  & Bestick et al. \cite{Bestick2017}      & \checkmark &   &   & \checkmark   & \checkmark  &  & \cellcolor[HTML]{FFFFFF}Fixed      & \checkmark   &  &    & \checkmark    & \checkmark    &     & \checkmark  \\
\hline
2017  & Peternel et al. \cite{Peternel2017}     & \checkmark &   &   & & \checkmark  &  & Fixed  & \checkmark   &  &    &      &      & \checkmark   &    \\
\hline
2017  & Konstantinova et al. \cite{Konstantinova2017}      & \checkmark & \checkmark &   & &    &  & Unclear & \checkmark   & \checkmark&    &      & \checkmark    &     &    \\
\hline
2018  & Controzzi et al. \cite{Controzzi2018}    & \checkmark &   &   & &    &  & Fixed  & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2018  & Pan et al.  \cite {Pan2018}   & & \checkmark   & \checkmark & \checkmark   & \checkmark  & \checkmark& \cellcolor[HTML]{FFFFFF}Not-fixed    & \checkmark   & \checkmark&    &      & \checkmark    &     & \checkmark  \\
\hline
2020      & Yang et al.  \cite {Yang2020}  & & \checkmark   &   & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  &    &      & \checkmark    &     & \checkmark  \\
\hline
2020      & Rosenberger et al.  \cite {Rosenberger2020}  & & \checkmark   &   & \checkmark   & \checkmark  & \checkmark& Not-fixed    & \checkmark   &  & \checkmark    &      & \checkmark    &     &   \\
\hline
\rowcolor[HTML]{E7E6E6} 
2006      & Kulic et al. \cite{Kulic2006}  & &   &   & & \checkmark  &  &     &     &  &    &      &      & \checkmark   & \checkmark  \\
\hline
\rowcolor[HTML]{E7E6E6} 
2009      & Bartneck et al. \cite{Bartneck2009}      & &  &   & &    &  &     &     &  &    &      &      &     & \checkmark  \\
\hline
\rowcolor[HTML]{E7E6E6} 
2019      & Hoffman \cite{Hoffman2019}    & &   &   & &    &  &     &     &  &    &      & \checkmark    &     & \checkmark \\
\hline
\end{tabular}
\caption{Comparison of the papers presenting novelty about human-robot handovers and experiments with a real system. This table reports: the paradigm (robot-to-human R2H or human-to-robot H2R); the aspects of the pre-handover phase under investigation (communication, grasping, motion planning and control, perception); whether the handover location was fully pre-planned (fixed) or adapted online (not-fixed); whether during the physical handover, grip force was regulated and error handling dealt with; whether the experimental protocol foresaw a post-handover task. Finally, we report whether the reported results are based on metrics encompassing the overall performance, and a quantitative and qualitative assessment of the experience of the human partner. The last three entries are papers purely investigating the metrics for a handover.}
\end{table}
\label{table:comparison}
\end{landscape}

==> table2.tex <==
\begin{landscape}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\centering
\begin{tabular}{? c ? l ? c | c ?c|c|c|c? c ?c|c?c?c|c|c? c ?}
\hline
\rowcolor[HTML]{D0CECE}
\multicolumn{1}{? c ?}{}     & \multicolumn{1}{c?}{}   & \multicolumn{2}{c?}{Paradigm} & \multicolumn{4}{c?}{Pre-Handover}    & \multicolumn{1}{c?}{}     &  \multicolumn{2}{c?}{ Physical Handover}    & \multicolumn{1}{c?}{}      & \multicolumn{3}{c?}{ Metric} & \multicolumn{1}{ c ?}{}  \\
\cline{3-8} \cline{10-11} \cline{13-15}
\rowcolor[HTML]{D0CECE}
\multicolumn{1}{? c ?}{}     & \multicolumn{1}{c?}{ }   & \multicolumn{2}{c?}{}  & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{ }  & \multicolumn{1}{c|}{}    & \multicolumn{1}{c?}{}   & \multicolumn{1}{c?}{ }     & \multicolumn{1}{c|}{}     & \multicolumn{1}{c?}{ }   &   & \multicolumn{1}{c?}{}      & \multicolumn{2}{c?}{User Experience} & \multicolumn{1}{ c ?}{}\\
\cline{14-15} 
\rowcolor[HTML]{D0CECE}
\multicolumn{1}{? c ?}{\multirow{-3}{*}{\cellcolor[HTML]{D0CECE}Year}} & \multicolumn{1}{c?}{\multirow{-3}{*}{ \begin{tabular}[x]{@{}c@{}c@{}}Paper\end{tabular}}}     & \multicolumn{1}{c|}{\multirow{-2}{*}{\begin{tabular}[x]{@{}c@{}}R2H\end{tabular}}} &
\multicolumn{1}{c?}{\multirow{-2}{*}{ \begin{tabular}[x]{@{}c@{}}H2R\end{tabular}}} &
\multicolumn{1}{c|}{\multirow{-2}{*}{\begin{tabular}[x]{@{}c@{}}Comm.\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\begin{tabular}[x]{@{}c@{}}Grasping\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{ \begin{tabular}[x]{@{}c@{}}Motion\end{tabular}}} & \multicolumn{1}{c?}{\multirow{-2}{*}{\begin{tabular}[x]{@{}c@{}}Perception\end{tabular} }} & \multicolumn{1}{c?}{\multirow{-3}{*}{ \begin{tabular}[x]{@{}c@{}}Handover\\Location\end{tabular} }} & \multicolumn{1}{c|}{\multirow{-2}{*}{ \begin{tabular}[x]{@{}c@{}}Grip  Force \\ Modulation\end{tabular}}} & \multicolumn{1}{c?}{\multirow{-2}{*}{ \begin{tabular}[x]{@{}c@{}}Error\\Handling\end{tabular}}} & \multicolumn{1}{c?}{\multirow{-3}{*}{ \begin{tabular}[x]{@{}c@{}}Post\\Handover\\Task\end{tabular} }} & \multicolumn{1}{c?}{\multirow{-2}{*}{ \begin{tabular}[x]{@{}c@{}}Task\\Performance\end{tabular}}} & Physiological     & Subjective &
\multicolumn{1}{ c ?}{\multirow{-3}{*}{ \begin{tabular}[x]{@{}c@{}}\# of\\Test\\Objects\end{tabular} }}
\\
\hline
%1997  & Agah et al. \cite{Agah1997} & R2H &  &  & \checkmark & \checkmark& Not-fixed  &  &  &  &  &  & & \\
%\hline
2007  & Edsinger\cite{Edsinger2007} & \checkmark & \checkmark & \checkmark& \checkmark & \checkmark & \checkmark& Pre-planned &  &  & \checkmark & \checkmark & & & 1\\
\hline
\rowcolor[HTML]{f0f0f5}
2009  & Choi\cite{Choi2009} & \checkmark & & \checkmark & & \checkmark & \checkmark& Pre-planned  &  &  &  & \checkmark &  & \checkmark  & 3\\
\hline
2009  & Huber\cite{Huber2009a}  & \checkmark &  &  & & \checkmark  &  & Fixed  & & & & & & \checkmark & 1\\
\hline
\rowcolor[HTML]{f0f0f5}
2010  & Sisbot\cite{Sisbot2010} & \checkmark & &  & & \checkmark & \checkmark& Pre-planned  &  &  &   & &  & & 1 \\
\hline
2011  & Dehais\cite{Dehais2011}  & \checkmark &   &   & & \checkmark  & \checkmark& Pre-planned  &  &  &  &  & \checkmark & \checkmark & 1\\
\hline
\rowcolor[HTML]{f0f0f5}
2011  & Cakmak\cite{Cakmak2011a} & \checkmark &  & \checkmark & & \checkmark  &  & Pre-planned &  &  &  &  &  & \checkmark & 5 \\
\hline
2011  & Cakmak\cite{Cakmak2011b} & \checkmark & & \checkmark& & \checkmark  &  & Fixed  &  &  &  & \checkmark &  & \checkmark & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2011  & Micelli\cite{Micelli2011} & & \checkmark  & & \checkmark & \checkmark& \checkmark& Pre-planned  &  &  &  & \checkmark & & \checkmark & 2 \\
\hline
2011  & Bohren\cite{Bohren2011} & \checkmark &   &   & \checkmark   & \checkmark  & \checkmark& Fixed   &  &   &   & \checkmark  &   & & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2012  & Mainprice\cite{Mainprice2012} & \checkmark &   &   & & \checkmark  & \checkmark& Pre-planned  &  &    &  & \checkmark    &     & \checkmark & 2 \\
\hline
2012  & Aleotti\cite{Aleotti2012}  & \checkmark &   &   & \checkmark   & \checkmark  & \checkmark& Pre-planned  &   &    &  & \checkmark  &     & \checkmark & 2 \\
\hline
\rowcolor[HTML]{f0f0f5}
2013  & Chan\cite {Chan2013}  & \checkmark &   &   & &  &  & Fixed  & \checkmark&    &      & \checkmark    &     & \checkmark & 1 \\
\hline
2013  & Shi\cite{Shi2013}   & \checkmark &   & \checkmark &    & \checkmark  & \checkmark& Online    &  &    &      & \checkmark    &     &   & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2013  & Yamane\cite {Yamane2013}  & & \checkmark   &   & & \checkmark  & \checkmark & Online   &  &    &      &      &     &   & 1 \\
\hline

%2013  & Strabala\cite{Strabala2013}  & \checkmark & \checkmark  & \checkmark & & \checkmark  & \checkmark& Not-fixed   & \checkmark&    &   & \checkmark   &     & \checkmark & 10 \\
%\hline

%\rowcolor[HTML]{f0f0f5}
2013  & Grigore\cite{Grigore2013}      & \checkmark &   & \checkmark & & \checkmark  & \checkmark& Fixed  &  &    &      & \checkmark    &     &     & 1\\
\hline
\rowcolor[HTML]{f0f0f5}
2014  & Aleotti\cite{Aleotti2014}      & \checkmark &   & \checkmark & \checkmark   & \checkmark  & \checkmark& Pre-planned  &  &    &      & \checkmark    &     & \checkmark & 3 \\
\hline
%\rowcolor[HTML]{f0f0f5}
2014  & Moon\cite{Moon2014}  & \checkmark &   & \checkmark & &    &  & Fixed  & &    &      & \checkmark    &     & \checkmark  & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2014  & Koene\cite{Koene2014} & \checkmark & \checkmark   & \checkmark & \checkmark   & \checkmark  & \checkmark& Online    & \checkmark&    &      & \checkmark    &     & \checkmark  & 1\\
\hline
2014  & Prada\cite{Prada2014}   & \checkmark & \checkmark   & \checkmark & \checkmark   & \checkmark  & \checkmark& Online    & &    &      & \checkmark    &     & \checkmark  & 1\\
\hline
\rowcolor[HTML]{f0f0f5}
2014  & Koene\cite{Koene2014b} & \checkmark & \checkmark   & \checkmark & \checkmark   & \checkmark  & \checkmark& Online    & &    & \checkmark     & \checkmark    &     & \checkmark &1 \\
\hline
2014  & Chan\cite{Chan2014b}  &  \checkmark &  &   &\checkmark &   &  & Fixed  & \checkmark &    &    &  \checkmark  &     &  & 1  \\
\hline
\rowcolor[HTML]{f0f0f5}
2014  & Chan\cite{Chan2014}  & \checkmark &   &   &\checkmark &  & \checkmark& Fixed  & &    &    \checkmark  &     &     &  & 3  \\
\hline
2015  & Admoni\cite{Admoni2014}       & \checkmark &   & \checkmark & & \checkmark  & & Fixed  & \checkmark&    & \checkmark    & \checkmark    &     & \checkmark & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2015  & Suay\cite{Suay2015}  & \checkmark &   &   & & \checkmark  & \checkmark& Pre-planned    &  &    &      &   & \checkmark   & & 3    \\
\hline
2015  & Huang\cite{Huang2015}  & \checkmark &   & \checkmark & &    & \checkmark& Fixed  &  &    &  \checkmark    & \checkmark    &     & \checkmark & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2016  & Parastegari\cite{Parastegari2016}  & \checkmark &   &   & &    & \checkmark& Fixed  & \checkmark& \checkmark  &      & \checkmark    &     & \checkmark & 1 \\
\hline
2016  & Maeda\cite{Maeda2016}  & \checkmark & \checkmark   &   & & \checkmark  & \checkmark& Online    &  &    & \checkmark    & \checkmark    &     &   & 4 \\
\hline
\rowcolor[HTML]{f0f0f5}
2016  & Vahrenkamp\cite{Vahrenkamp2016}   & \checkmark &      &   & \checkmark   & \checkmark  & \checkmark& Online    &  &    &      &     &     &  & 1  \\
\hline
2016  & Kupcsik\cite{Kupcsik16}      & \checkmark &   &   & & \checkmark  & \checkmark& Fixed    & \checkmark&    &      &      &     & \checkmark & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2016  & Medina\cite{Medina2016}       & \checkmark &    &   & & \checkmark  & \checkmark& Online    &  &    &      & \checkmark    &     & & 1   \\
\hline
2017  & Eguiluz \cite{Gomez2017} & \checkmark & & &  & & & Fixed & \checkmark& \checkmark &  & \checkmark&  &  & 3\\
\hline
\rowcolor[HTML]{f0f0f5}
2017  & Bestick\cite{Bestick2017}      & \checkmark &   &   & \checkmark   & \checkmark  &  & Pre-planned      &  &    & \checkmark    & \checkmark    &     & \checkmark & 1 \\
\hline
2017  & Peternel\cite{Peternel2017}     & \checkmark &   &   & & \checkmark  &  & Online  &  &    &      &      & \checkmark   &  & 1  \\
\hline
\rowcolor[HTML]{f0f0f5}
2017  & Konstantinova\cite{Konstantinova2017}      & \checkmark & \checkmark &   & &    &  &  Fixed & \checkmark&    &      & \checkmark    &     &    & $>$6\\
\hline
2018  & Controzzi\cite{Controzzi2018}    & \checkmark &   &   & &    &  & Fixed  & \checkmark&    &      & \checkmark    &     & \checkmark & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2018  & Pan\cite {Pan2018}   & & \checkmark   & \checkmark & \checkmark   & \checkmark  & \checkmark& Online    & \checkmark& \checkmark    &      & \checkmark    &     & \checkmark & 1 \\
\hline
2020      & Yang\cite {Yang2020}  & & \checkmark   &   & \checkmark   & \checkmark  & \checkmark& Pre-planned    &  &    &      & \checkmark    &     & \checkmark  & 1 \\
\hline
\rowcolor[HTML]{f0f0f5}
2020      & Rosenberger\cite {Rosenberger2020}  & & \checkmark   &   & \checkmark   & \checkmark  & \checkmark& Pre-planned    &  &     &      & \checkmark    &     & & 13   \\
\hline
\rowcolor[HTML]{E7E6E6} 
2006      & Kulic\cite{Kulic2006}  & &   &   &  &  &     &     &  &    &      &      & \checkmark   & \checkmark & \\
\hline
\rowcolor[HTML]{E7E6E6} 
2009      & Bartneck\cite{Bartneck2009}      &&   & &    &  &     &     &  &    &      &      &     & \checkmark  &\\
\hline
\rowcolor[HTML]{E7E6E6} 
2019      & Hoffman\cite{Hoffman2019}    & &   &   &    &  &     &     &  &    &      & \checkmark    &     & \checkmark &\\
\hline
\end{tabular}
\caption{Comparison of the papers presenting novelty about human-robot handovers and experiments with a real system. This table reports: the paradigm (robot-to-human R2H or human-to-robot H2R); the aspects of the pre-handover phase under investigation (communication, grasping, motion planning and control, perception); whether the handover location was fixed or fully pre-planned or adapted online; whether grip force was regulated and error handling dealt with during the physical handover; whether the experimental protocol foresaw a post-handover task; which metrics were utilised for the evaluation of the experiments (task metric, physiological, subjective); and how many objects were used in the handover tests.}
\end{table}
\vspace{10pt}
\label{table:comparison}
\end{landscape}

==> table_none.tex <==
\begin{landscape}
\begin{table}
    \centering
    \centering
\begin{tabular}{? c ? c | c ? c | c | c | c ? c ? c | c | c ?c?c|c|c? c ?}
\hline
    
   % \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
    \rowcolor[HTML]{D0CECE}
         & \multicolumn{2}{c?}{Paradigm}  & \multicolumn{4}{c?}{Pre-Handover} & Handover & \multicolumn{3}{c?}{Physical Handover} & Post-HO & \multicolumn{3}{c?}{Metrics} & Test\\
        \rowcolor[HTML]{D0CECE}
         Paper & R2H & H2R & Comm. & Grasping & Motion & Perception &  Location & Perception & Grip Force & Error & Task & Task performance & \multicolumn{2}{c?}{User experience} &  Objects\\ 
         \rowcolor[HTML]{D0CECE}
         &  &  &  &  & &  &  &  &  & handling &  &  & Physiological & Subjective &  \\ \hline
         \rowcolor[HTML]{f0f0f5}
        \cite{Huber2009} & YES &  &  &  & YES & - & Fixed & force torque sensors &  &  &  &  &  & questionnaire & 1 \\ \hline
        \cite{Chan2013} & YES &  &  &  &  & - & Fixed & {\begin{tabular}{c}Pressure sensors,\\ 6-axis force/torque sensor,\\ force sensing resistors\end{tabular}} & YES & &  & {\begin{tabular}{c}grip force, load force,\\ transfer time,\\ maximum load transfer rate\end{tabular}} &  & questionnaire & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Chan2014b} & YES &  &  & YES &  & - & Fixed & Force sensor & YES &  &  & {\begin{tabular}{c}timing, maximum excess\\ receiver load force\end{tabular}} &  &  & 1  \\ \hline
        \cite{Parastegari2016} & YES &  &  &  &  & optical sensor & Fixed & Force sensor & YES & YES &  & forces &  & questionnaire & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Gomez2017} & YES &  &  &  &  & - & Fixed & tactile sensors & YES & YES &  & forces &  &  & 3 \\ \hline
        \cite{Konstantinova2017} & YES & YES &  &  &  & - & Fixed & force/torque sensor & YES &  &  & forces, jerk &  &  & $>$6  \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Controzzi2018} & YES &  &  &  &  & - & Fixed & force/torque sensor & YES &  &  & timing, acceleration, forces &  & questionnaire & 1 \\ \hline
        \cite{Han2019} & YES &  & YES & YES & YES & - & Online &  {\begin{tabular}{c}force sensor,\\ force sensing resistor\end{tabular}} & YES &  & YES & completion time &  & questionnaire & 1  \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Davari2019} & YES &  &  &  &  & - & Fixed & Tactile sensors &  & YES &  &  &  &  & 3 \\ \hline
        \cite{Ortenzi2020} & YES &  &  & YES &  & - & Fixed & force/torque sensor &  &  & YES & {\begin{tabular}{c}timing, post-handover\\ readjustments\end{tabular}} &  & questionnaire & 5\\ \hline
    \end{tabular}
\caption{Force as main perception modality.}
\label{table:force}
\end{table}
\begin{table}
    \centering
\begin{tabular}{? c ? c | c ? c | c | c | c ? c ? c | c | c ?c?c|c|c? c ?}
    \hline
    \rowcolor[HTML]{D0CECE}
         & \multicolumn{2}{c?}{Paradigm}  & \multicolumn{4}{c?}{Pre-Handover} & Handover & \multicolumn{3}{c?}{Physical Handover} & Post-HO & \multicolumn{3}{c?}{Metrics} & Test\\
        \rowcolor[HTML]{D0CECE}
         Paper & R2H & H2R & Comm. & Grasping & Motion & Perception &  Location & Perception & Grip Force & Error & Task & Task performance & \multicolumn{2}{c?}{User experience} &  Objects\\ 
         \rowcolor[HTML]{D0CECE}
         &  &  &  &  & &  &  &  &  & handling &  &  & Physiological & Subjective &  \\ \hline
         \rowcolor[HTML]{f0f0f5}
        \cite{Edsinger2007} & YES & YES & YES & YES & YES & - & Pre-planned & - &  &  & YES & {\begin{tabular}{c}failures, grasp alignment error\end{tabular}} &  &  & 1 \\ \hline
         \cite{Fujita2010} & YES &  &  &  & YES & - & Fixed & - &  &  &  &  & skin potential response & questionnaire & 1 \\ \hline
         \rowcolor[HTML]{f0f0f5}
        \cite{Cakmak2011a}  & YES &  & YES &  & YES & - & Pre-planned & - &  &  &  &  &  & questionnaire & 5 \\ \hline
        \cite{Cakmak2011b}  & YES &  & YES &  & YES & - & Fixed & - &  &  &  &{\begin{tabular}{c} human waiting time, \\robot waiting time, fluency\end{tabular}}  &  & questionnaire & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Moon2014} & YES &  & YES &  &  & - & Fixed & - &  &  &  & timing &  & questionnnaire & 1 \\ \hline
        \cite{Admoni2014} & YES &  & YES &  & YES & - & Fixed & - & YES &  & YES & rate of participant compliance &  & questionnaire & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Maeda2016} & YES & YES &  &  & YES & - & Online & - &  &  & YES & success rate &  &  & 4 \\ \hline
        \cite{Vahrenkamp2016} & YES &  &  & YES & YES & - & Online & Force sensor &  &  &  &  &  &  & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Bestick2017} & YES &  &  & YES & YES & - & Pre-planned & - &  &  & YES & estimated ergonomic cost &  & questionnaire & 1 \\ \hline
        \cite{Bianchi2018} &  & YES &  & YES &  & IMU & Pre-planned & - &  &  &  & Success rate &  &  & 22 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Sanchez-Matilla2020} &  & YES &  & YES & YES & YES & Fixed* &  &  &  & YES & YES &  &  & 4 \\ \hline
    \end{tabular}
\caption{No sensor used for perception during any phase.}
\label{table:nosensor}
\end{table}
\begin{table}
    \centering
\begin{tabular}{? c ? c | c ? c | c | c | c ? c ? c | c | c ?c?c|c|c? c ?}
    \hline
    \rowcolor[HTML]{D0CECE}
         & \multicolumn{2}{c?}{Paradigm}  & \multicolumn{4}{c?}{Pre-Handover} & Handover & \multicolumn{3}{c?}{Physical Handover} & Post-HO & \multicolumn{3}{c?}{Metrics} & Test\\
        \rowcolor[HTML]{D0CECE}
         Paper & R2H & H2R & Comm. & Grasping & Motion & Perception &  Location & Perception & Grip & Error & Task & Task performance & \multicolumn{2}{c?}{User experience} &  Objects\\ 
         \rowcolor[HTML]{D0CECE}
         &  &  &  &  & &  &  &  & Force & handling &  &  & Physiological & Subjective &  \\ \hline
         \rowcolor[HTML]{f0f0f5}
         \cite{Choi2009} & YES &  & YES &  & YES & {\begin{tabular}{c}  laser pointer, camera,\\ laser range ﬁnder\end{tabular}} & Pre-planned & {\begin{tabular}{c}  force-sensing ﬁngers,\\ 6-axis force plate\end{tabular}} &  &  &  & {\begin{tabular}{c}detection time, transport time,\\ placing/handing time, grasping time,\\ total time, failures, success rate\end{tabular}} &  & questionnaire & 3 \\ \hline
         \cite{Kupcsik16} & YES &  &  &  & YES & Kinect camera (RGBD) & Fixed & Force sensor & YES &  &  &  &  & questionnaire & 1 \\ \hline
         \rowcolor[HTML]{f0f0f5}
         \cite{Medina2016} & YES &  &  &  & YES & motion capture & Online & force/torque sensor &  &  &  & forces, timing &  &  & 1 \\ \hline
         \cite{Peternel2017} & YES &  &  &  & YES & IMU suit &  Online & force/torque sensor &  &  &  &  & EMG &  & 1 \\ \hline
         \rowcolor[HTML]{f0f0f5}
         \cite{Meyer2017} & YES & YES & YES &  & YES & Camera &  Fixed & Force sensor & YES &  & ? & {\begin{tabular}{c}movement speed, reaction time,\\ manipulation time\end{tabular}} &  & questionnaire & 3 \\ \hline
         \cite{Pan2018} &  & YES & YES & YES & YES & motion capture &  Online & force/torque sensor & YES & YES &  & forces, &  & questionnaire & 1 \\ \hline
    \end{tabular}
\caption{Vision and Force as main perception modalities.}
\label{table:visionforce}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
    \centering
\begin{tabular}{? c ? c | c ? c | c | c | c ? c ? c | c | c ?c?c|c|c? c ?}
    \hline
    \rowcolor[HTML]{D0CECE}
         & \multicolumn{2}{c?}{Paradigm}  & \multicolumn{4}{c?}{Pre-Handover} & Handover & \multicolumn{3}{c?}{Physical Handover} & Post-HO & \multicolumn{3}{c?}{Metrics} & Test\\
        \rowcolor[HTML]{D0CECE}
         Paper & R2H & H2R & Comm. & Grasping & Motion & Perception &  Location & Perception & Grip & Error & Task & Task performance & \multicolumn{2}{c?}{User experience} &  Objects\\ 
         \rowcolor[HTML]{D0CECE}
         &  &  &  &  & &  &  &  & force & handling &  &  & Physiological & Subjective &  \\ \hline
         \rowcolor[HTML]{f0f0f5}
        \cite{Dehais2011} & YES &  &  &  & YES & {\begin{tabular}{c} sonars,\\ two laser range ﬁnders,\\ two stereo camera banks\end{tabular}}  & Pre-planned & {\begin{tabular}{c}contact sensors,\\ a wrist force sensor\end{tabular}} &  &  &  &  & {\begin{tabular}{c}skin conductance,\\ deltoid muscle activity,\\ oculometry\end{tabular}} & questionnaire & 1 \\ \hline
        \cite{Micelli2011} &  & YES &  & YES & YES & Kinect camera (RGBD) & Pre-planned & 6-axis force-torque sensor &  &  &  & {\begin{tabular}{c}success rate,\\ completion time\end{tabular}} &  & questionnaire & 2 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Bohren2011} & YES &  &  & YES & YES & tilting laser, stereo camera  & Fixed & - &  &  &  & completion time &  &  & 1 \\ \hline
        \cite{Aleotti2012} & YES &  &  & YES & YES & {\begin{tabular}{c}laser scanner,\\   Kinect camera (RGBD)\end{tabular}} & Pre-planned & - &  &  &  & {\begin{tabular}{c}perception time,\\ completion time\end{tabular}} &  & questionnnaire & 2 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Mainprice2012} & YES &  &  &  & YES & camera, & Pre-planned & - &  &  &  & timing &  & questionnnaire & 2 \\ \hline
        \cite{Sisbot2013} & YES &  &  &  & YES & camera & Pre-planned & force sensor &  &  &  &  &  &  & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Shi2013} & YES &  & YES &  & YES & 3D range senrors, cameras &  Online & - &  &  &  & success rate &  &  & 1 \\ \hline
        \cite{Yamane2013} &  & YES &  &  & YES & motion capture &  Online & - &  &  &  &  &  &  & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Grigore2013} & YES &  & YES &  & YES & motion capture & Fixed & - &  &  &  & success rate &  &  & 1 \\ \hline
        \cite{Aleotti2014} & YES &  & YES & YES & YES & {\begin{tabular}{c}laser scanner,\\   Kinect camera (RGBD)\end{tabular}} &  Pre-planned & - &  &  &  & success rate, timing &  & questionnaire & 3 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Koene2014} & YES & YES & YES & YES & YES & Kinect camera (RGBD) & Online & capacitive touch sensors & YES &  &  & success rate &  & questionnaire & 1 \\ \hline
        \cite{Prada2014} & YES & YES & YES & YES & YES & Kinect camera (RGBD) & Online & - &  &  &  & success rate &  & questionnaire & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Koene2014b} & YES & YES & YES & YES & YES & Kinect camera (RGBD) & Online & - &  &  & YES & ? &  & questionnaire & 1 \\ \hline
        \cite{Chan2014b} & YES &  &  & YES &  & motion capture &  Fixed & - &  &  & YES &  &  &  & 3 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Unhelkar2014} & YES &  & YES &  & YES & Laser scanner, RGBD & Fixed & - &  &  & YES & {\begin{tabular}{c}interaction time,\\ assistant idle time\end{tabular}} &  & questionnaire & 3* \\ \hline
        \cite{Suay2015} & YES &  &  &  & YES & Kinect camera (RGBD) & Pre-planned & - &  &  &  &  & {\begin{tabular}{c}electromyogram\\ (EMG)\end{tabular}}  &  & 3 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Huang2015} & YES &  & YES &  &  & Kinect camera (RGBD) & Fixed & force sensor &  &  & YES & {\begin{tabular}{c}task completion time,\\ concurrent activity,\\ user idle time,\\ robot idle time\end{tabular}} &  & questionnaire & 1 \\ \hline
        \cite{Quispe2017} & YES &  & YES &  & YES & RGBD, rangefinder & Pre-planned & - &  &  &  &  &  & questionnaire & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Wu2019} &  & YES &  &  & YES & motion capture & Online & - &  &  &  &  &  &  &  \\ \hline
        \cite{Sidiropoulos2019} & YES &  &  &  & YES & Kinect camera (RGBD) & Online & - & YES &  &  &  &  &  & 1 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Yang2020} &  & YES &  & YES & YES & RGBD &  Pre-planned & - &  &  &  &  {\begin{tabular}{c}success rate,\\ detection rate,\\ timing\end{tabular}}  &  & questionnaire & 1 \\ \hline
        \cite{Rosenberger2020} &  & YES &  & YES & YES & RGBD & Pre-planned & - &  &  &  & success rate &  &  & 13 \\ \hline
        \rowcolor[HTML]{f0f0f5}
        \cite{Ardon2020} & YES &  &  & YES & YES & Camera? & Pre-planned & - &  &  & YES & accuracy &  &  & 10 \\ \hline
        \cite{Yang2020reactive} &  & YES &  & YES & YES & RGBD & Pre-planned & - &  &  &  & {\begin{tabular}{c}completion time,\\ grasp attempts,\\  success rate,\\ approach time\end{tabular}} &  & {\begin{tabular}{c}questionnaire,\\ open questions\end{tabular}} & 26 \\ \hline
    \end{tabular}
\caption{Vision  as main perception modality.}
\label{table:vision}
\end{table}
\end{landscape}
